Complexity of Deliberative Coalition Formation

Elkind et al. (AAAI, 2021) introduced a model for deliberative coalition formation, where a community wishes to identify a strongly supported proposal from a space of alternatives, in order to change the status quo. In their model, agents and proposals are points in a metric space, agents' preferences are determined by distances, and agents deliberate by dynamically forming coalitions around proposals that they prefer over the status quo. The deliberation process operates via k-compromise transitions, where agents from k (current) coalitions come together to form a larger coalition in order to support a (perhaps new) proposal, possibly leaving behind some of the dissenting agents from their old coalitions. A deliberation succeeds if it terminates by identifying a proposal with the largest possible support. For deliberation in d dimensions, Elkind et al. consider two variants of their model: in the Euclidean model, proposals and agent locations are points in R^d and the distance is measured according to ||...||_2; and in the hypercube model, proposals and agent locations are vertices of the d-dimensional hypercube and the metric is the Hamming distance. They show that in the continuous model 2-compromises are guaranteed to succeed, but in the discrete model for deliberation to succeed it may be necessary to use k-compromises with k >= d. We complement their analysis by (1) proving that in both models it is hard to find a proposal with a high degree of support, and even a 2-compromise transition may be hard to compute; (2) showing that a sequence of 2-compromise transitions may be exponentially long; (3) strengthening the lower bound on the size of the compromise for the d-hypercube model from d to 2^{\Omega(d)}.

==> extra/euclid.tex <==
\section{Euclidean Deliberation Space}\label{sec:euclid}
In this section, we shall focus on a natural model where the space of proposals $\cX = \bR^d$, for some integer $d > 0$, the agents $\cV$ are a set of points in $\bR^d$, $|\cV| = n$, and the distance $\rho$ is defined using the Euclidean norm. For the ease of presentation, we shall assume $\rho(x,v) = ||x-v||_2^2$ instead of $||x-v||_2$; this does not have any affect of the agents' preferences. We shall also assume that the status quo is at the origin, $r = 0$, w.l.o.g.

For Euclidean spaces, the following is known from~\cite{elkind2021united}:
\begin{theorem}\cite{elkind2021united}\label{thm:euclidSuccess}
In every Euclidean deliberation space, every maximal run of $2$-compromise transitions is a successful deliberation, and there exists a sequence of $2$-compromise transitions that terminates after $(n^2+1)$ steps.
\end{theorem}
For the sequence that terminates in $(n^2+1)$ steps, as mentioned in the theorem above, they also sketch a method to find the $2$-compromise transitions in the sequence. 

\subsection{Complexity of Finding the Optimal Proposal}
Our first result shows that finding an optimal proposal (equivalently an optimal coalition structure) is NP-hard, which, as a direct corollary, shows that some of the $2$-compromise transitions in the sequence can be NP-hard to compute, and therefore, it may be difficult to realize the sequence in practice. On the other hand, the problem is fixed parameter tractable; if we assume that either $n$ or $d$ is a constant, then we can find an optimal proposal in polynomial time.

\begin{theorem}\label{thm:euclidNPHard}
In a Euclidean deliberation space, it is NP-complete to decide whether there exists a proposal that is supported by at least $\eta$ agents for some $\eta \in [n]$. ($n$ is polynomial in the number of dimensions $d$.)
\end{theorem}
We prove the above theorem by a reduction from 3-SAT; proof provided in the Appendix.

\begin{theorem}\label{thm:euclidFPT}
In a Euclidean deliberation space, if either the dimension of the space $d$ or the number of agents $n$ is a constant, an optimal proposal can be efficiently computed.
\end{theorem}
\begin{proof}[Theorem~\ref{thm:euclidFPT}] Given a proposal $p$ and an agent $v$, $v$ supports $p$ iff
\begin{equation}\label{eq:prf:euclidFPT}
    \rho(v,p) < \rho(v,0) \Longleftrightarrow || p ||^2 < 2 \langle v , p \rangle.
\end{equation}
So, a given proposal $p$ divides $\bR^d$ into two half-spaces; the half-spaces are divided by the hyper-plane orthogonal to and bisecting the line-segment joining $p$ to the origin. We shall use this correspondence between proposals and half-spaces in the proof.

\textit{Constant number of agents.} For every subset $S \subseteq \cV$ of agents, we check whether there is a hyper-plane passing through the origin that has all the agents in $S$ strictly on one side of the hyper-plane. This can be done efficiently by checking whether there exists an $x \in \bR^d$ that satisfies the following linear program: $\langle v , x \rangle > 0, \forall v \in S$. Once we find such an $x$, we can set the proposal $p = \epsilon x / ||x|| $ for a very small $\epsilon > 0$. As $n = |\cV|$ is a constant, repeating this process for every $S \subseteq \cV$ is not an issue (which is at most $2^n$ times, a constant).

\textit{Constant number of dimensions.} As we observed earlier, a proposal divides $\bR^d$ into two half-spaces. The set of half-spaces in $\bR^d$ has a VC-dimension of $(d+1)$~\cite{kearns1994introduction}, and therefore, the set of proposals also has a VC-dimension of at most $(d+1)$. Given a set $\cV$ of $n$ agents, let $\cS$ be the following set of subsets of agents:
\[ 
    \cS = \{ S \subseteq \cV \mid \exists x \in \cX \text{ s.t. $|| x ||^2 < 2 \langle v , x \rangle, \forall v \in S$ and $|| x ||^2 
    \ge 2 \langle v , x \rangle, \forall v \notin S$} \}.
\]
In other words, for every set $S \in \cS$, there exists a proposal that is supported by all the agents in $S$ and none of the agents not in $S$. As the set of proposals has a VC-dimension of $(d+1)$, the set $\cS$ has a size of $O(n^{d+1})$ and the elements of $\cS$ can be enumerated in time polynomial in $n$.\footnote{See Lemma~3.1 and 3.2 of Chapter 3 of the book by Kearns and Vazirani~\cite{kearns1994introduction}. The elements of $\cS$ can be computed inductively, see the proof of Lemma~3.1. We are also using the fact that given an arbitrary set of agents $S$, we can efficiently compute a proposal that is supported by exactly the agents in $S$ by solving an LP, as we did for constant number of agents.} So, we can find the largest $S$ in $\cS$ and the corresponding proposal efficiently.
\qed\end{proof}

% \abheek{TODO: For constant $d$ and arbitrary $n$, what can we say about the complexity of the problem? This can be answered if we get the answer of: Can we list all subsets of a set $S$ in $\bR^d$ \textit{realized} by half-spaces in time polynomial in $|S|$?}

\subsection{Slow Convergence of Compromise Transitions}\label{sec:euclidSlow}
The other important question for Euclidean deliberation spaces is whether all sequences of $2$-compromise transitions terminate after a number of steps polynomial in $n$? Theorem~\ref{thm:euclidSuccess} gives a sequence that does terminate quickly in $(n^2+1)$ steps, but the only known upper bound is $n^n$, given in Theorem~\ref{thm:compromisenn}, proved using a lexicographic potential function. In the next theorem, we slightly improve this upper bound to $2^n$. 
% (Proof of Theorem~\ref{thm:compromiseUpperBd} is provided in the Appendix.)
\begin{theorem}\label{thm:compromiseUpperBd}
$2$-compromise transitions converge in at most $2^n$ steps, which can be showed using the following potential function \begin{equation}\label{eq:potential2Compromise}
    \phi(\cC) = - |\cC| + \sum_{C \in \cC} 2^{|C|},
\end{equation}
where $\cC$ is the set of non-empty coalitions in a coalitions structure, and $\phi(\cC)$ is its potential value.
\end{theorem}
\begin{proof} %[Theorem~\ref{thm:compromiseUpperBd}]
Let $\cC$ be the set of non-empty coalitions in a coalitions structure. 
% As given in the theorem statement, the potential function $\phi$ is defined as:
% \begin{equation*}
%     \phi(\cC) = - |\cC| + \sum_{C \in \cC} 2^{|C|}.
% \end{equation*}
Note that $\bigcup_{C \in \cC} = \cV$ (an isolated agent is in its own singleton coalition).

Say a $2$-compromise transition occurs, where two coalitions $A$ and $B$ of sizes $a$ and $b$ in $\cC$ compromise to form coalitions $C$, $D$, and $E$ of sizes $c$, $d$ and $e$ in $\cC'$. W.l.o.g, $a \le b < c$ and $c \ge d \ge e$. Note that $D$ and $E$ may be empty, and then would not be included in the new set of non-empty coalitions $\cC'$ and the potential $\phi(\cC')$ ($d$ and $e$ would not exist). We know that $a + b = c + d + e$, and the value of $|\cC'| - |\cC|$ may be either $-1$, $0$ , or $1$, depending upon whether $D$ and $E$ are empty. 

The change in potential is $\phi(\cC') - \phi(\cC) = 2^c - 2^a - 2^b + 1 + (2^d - 1) + (2^e - 1)$ where $(2^d - 1)$ and $(2^e - 1)$ apply iff $D$ and $E$ are non-empty, respectively. In other words, if $D$ is non-empty then it contributes $2^d$ to the $\sum_{C \in \cC'} 2^{|C|}$ and $-1$ to the $-|\cC'|$ portion of $\phi(\cC')$, if $D$ is empty then neither of these are present in $\phi(\cC')$. As $(2^d - 1)$ and $(2^e - 1)$ are always non-negative, we get
\[ \phi(\cC') - \phi(\cC) \ge 2^c - 2^a - 2^b + 1 \ge 2*2^b - 2^b - 2^b + 1 = 1, \]
as $c > b \ge a$. So, any compromise transition increases the potential by at least $1$. It is easy to check that $n \le \phi(\cC) \le 2^n - 1$ for any $\cC$.

% We repeatedly use the fact that $(2^d - 1)$ and $(2^d - 1)$ are always non-negative; on a case by case basis, the change in potential is:
% \begin{itemize}
%     \item If $c > b+1$, then $\phi(\cC') - \phi(\cC) \ge 2^c - 2^a - 2^b + 1 \ge 4*2^b - 2^a - 2^b + 1 \ge 2*2^b+1 \ge 1$. 
%     \item If $c = b+1$ and $a = 1$, then $\phi(\cC') - \phi(\cC) = 2*2^b - 2^a - 2^b + 1 \ge 1$.
%     \item If $c = b+1$ and $a \ge 2$, then $\phi(\cC') - \phi(\cC) \ge 2*2^b + 2^d - 2^a - 2^b - 1 \ge 2^d - 1 \ge 1$.
% \end{itemize}
\qed\end{proof}
Observe that the above theorem is independent of the deliberation space and is a property of $2$-compromise transitions. A similar result can be proven for $k$-compromise transitions: they converge in at most $k^n$ steps.

We now focus on lower bound on the convergence of $2$-compromise transitions. We do it in two steps: first, we prove a lemma that applies to any deliberation space that satisfies a certain property; then, we give an example of a Euclidean deliberation space where the property holds. The lemma will also be useful for hypercube deliberation spaces.

\begin{lemma}\label{thm:compromiseSlowConverg}
If a deliberation space with the set of proposals $\cX$ and the set of agents $\cV$ satisfies the following property: for every $C \subseteq \cV$ there exists a proposal $p \in \cX$ s.t. all the agents in $C$ support $p$ and none of the agents not in $C$ support $p$; then, a deliberation may take $\Omega(2^{\sqrt{n}/2})$ $2$-compromise transitions.
\end{lemma}
\begin{proof}
The property of the deliberation space mentioned in the theorem statement implies that any $2$-compromise transition that leads to a strictly larger coalition is valid, i.e., for a given transition, we need not worry whether there is a proposal that is supported by all the agents that form the new coalition and not supported by any of the agents that were left behind, because such a proposal always exists.

Let $\cC$ be the set of non-empty coalitions in a coalition structure. We now prove that if the agents end up executing the following types of $2$-compromise transitions, then they will take an exponential time to converge, starting from the coalition structure where all the agents are in singleton coalitions.
\begin{enumerate}
    \item \textbf{Type 1.} If there is a pair $C,C' \in \cC$ s.t. $|C| = |C'|$, then make the following transition (written using coalition sizes):
    \begin{equation}\label{eq:move1}
        (a) + (a) \longrightarrow (a+1) + (\floor{\frac{a-1}{2}}) + (\ceil{\frac{a-1}{2}}),
    \end{equation}
    where $a = |C| = |C'|$. The change in potential (as defined in \eqref{eq:potential2Compromise}) for such a transition is
    \begin{align}\label{eq:potentialChangeType1}
        \Delta \Phi &\le 2^{a+1} + 2^{\floor{\frac{a-1}{2}}} + 2^{\ceil{\frac{a-1}{2}}} - 2*2^{a} = 2^{\floor{\frac{a-1}{2}}} + 2^{\ceil{\frac{a-1}{2}}} \le \frac{3}{2} 2^{a/2}. % & \text{ if $a$ odd, then $= \sqrt{2} 2^{a/2} \le \frac{3}{2} 2^{a/2} $ }
    \end{align}
    (Note that $(\floor{\frac{a-1}{2}})$ and $(\ceil{\frac{a-1}{2}})$ may be $0$, which implies that the number of coalitions decreases, and therefore, may contribute $1$ to $\Delta \phi$ due to change in $|\cC|$. But, in that case $2^{\floor{\frac{a-1}{2}}}$ wouldn't be in $\Delta \Phi$, so they compensate.)
    \item \textbf{Type 2.} If there are no Type 1 transitions available, then select the two smallest coalitions $C,C' \in \cC$ and make the following transition:
    \begin{equation}\label{eq:move2}
        (a) + (b) \longrightarrow (b+1) + (\floor{\frac{a-1}{2}}) + (\ceil{\frac{a-1}{2}}),
    \end{equation}
    where $a = |C|$, $b = |C'|$ and $a \le b$. 
\end{enumerate}

Now, if $\max_{C \in \cC} |C| \le \sqrt{n}$, then there must be at least one pair of coalitions of same size. If not, then 
\[ \sum_{i=1}^{\sqrt{n}} i = \sqrt{n} (\sqrt{n}+1)/2 = n/2 + \sqrt{n}/2 < n, \]
for large enough $n$, we get a contradiction. So, only Type 1 transitions are made until $\max_{C \in \cC} |C|$ goes above $\sqrt{n}$.

From Equation~\ref{eq:potentialChangeType1}, until $\max_{C \in \cC} |C| \le \sqrt{n}$ holds, we know that the change in potential for Type 1 transitions is bounded by
\[ \Delta \Phi \le \frac{3}{2} 2^{a/2} \le \frac{3}{2} 2^{\sqrt{n}/2}.\]
We also know that if $\max_{C \in \cC} |C|$ goes above $\sqrt{n}$ then the value of $\phi$ must go above $2^{\sqrt{n}} - n$, and the initial value of $\phi$ is $n$. So, the number of transitions must be at least
\[ \frac{2}{3} \frac{2^{\sqrt{n}} - 2n}{2^{\sqrt{n}/2}} = \frac{2}{3} (2^{\sqrt{n}/2} - \frac{2n}{2^{\sqrt{n}/2}}) \]
\qed\end{proof}

\begin{theorem}\label{thm:euclidSlowConverg}
There exist Euclidean deliberation spaces where a deliberation may take $\Omega(2^{\sqrt{n}/2})$ $2$-compromise transitions.
\end{theorem}
% The proof it provided in the Appendix; it works by constructing an Euclidean deliberation space that satisfies the condition required for Lemma~\ref{thm:compromiseSlowConverg}.
\begin{proof} %[Theorem~\ref{thm:euclidSlowConverg}]
Let $d=n$, i.e., the Euclidean space be of $d = n = |\cV|$ dimensions. Let the agent $v_i \in \cV$ be positioned on the $i$-th axis at a distance of $1$ from the origin, i.e., agent $v_1$ is located at $(1,0, \ldots, 0)$, agent $v_2$ at $(0,1,0,\ldots,0)$, and so on. 

For every $S \subseteq \cV$, let the point $x^S$ be defined as
\[
x^S_i = \begin{cases} 1/|S|, & \text{ if $v_i \in S$} \\
0, & \text{ otherwise}
\end{cases}.
\]
Observe that the distance of agent $v_i \in S$ from $x^S$ is $\rho(v_i,x^S) = (1-1/|S|)^2 + (1/|S|)^2(|S|-1) = 1 - 1/|S| < 1$, so agent $v_i$ prefers $x^S$ to the status-quo. But, for an agent $v_i \notin S$, the distance of $v_i$ from $x^S$ is $1 + |S| (1/|S|)^2 = 1 + 1/|S| > 1$. So, for any subset of agents $S$, there is a proposal $x^S$ that is supported exactly by the agents in $S$. Applying Lemma~\ref{thm:compromiseSlowConverg}, we get the desired result.
\qed\end{proof}

==> extra/grid.tex <==
\section{2-Dimensional Grid}
In this section, we study a version of the coalition formation problem when all the players and proposals are located on a two dimensional grid. We study two variations of the problem: first, when all the players and proposals are points in the first quadrant $\bZ_{\ge 0}^2$, and the status quo is at $(0,0)$, we call this the $\bZ_{\ge 0}^2$ grid variation; and the more general second variation, when the players and proposals are points in $\bZ^2$, and w.l.o.g. the status quo is at $(0,0)$,  we call this the $\bZ^2$ grid variation. The distance is measured by $l_1$ norm, or equivalently, the shortest distance using the edges of the grid, where every point on the grid has four edges, one each to the left, right, up, and down.

The following two examples show that a 2-compromise is necessary for $\bZ_{\ge 0}^2$ grid and a 3-compromise is necessary for $\bZ^2$ grid. Later, we will show that it is sufficient.
\begin{enumerate}
    \item There are five players: two located at $(0,1)$, two at $(1,1)$, and one at $(1,0)$. The current coalition structure has two coalitions: first coalition consisting of the two players at $(0,1)$ with a proposal at $(0,1)$, and second coalition with the remaining three players with a proposal at $(1,0)$. For players at $(1,0)$, the only proposal the prefer to status quo is $(1,0)$, similarly, players at $(0,1)$ only prefer $(0,1)$, but the players at $(1,1)$ prefer proposals at both $(1,0)$ or $(0,1)$, among other proposals. It is easy to check that the optimal coalition structure has a coalition with four players with a proposal at $(0,1)$, but given the current situation, there are no single-agent or merge transitions that can lead to an optimal coalition structure. On the other hand, a compromise between the two current coalitions leads to an optimal coalition structure.
    
    \item There are nine players: one at $(1,0)$, and two at each of $(-1,0)$, $(-1,1)$, $(1,1)$, $(1,0)$. The current coalition structure has three coalitions: (a) players at $(-1,0)$ and $(-1,1)$ in a coalition of size four at $(-1,0)$; (b) players at $(1,0)$ and $(1,1)$ in a coalition of size four at $(1,0)$; (c) the player at $(0,1)$ in a coalition of size one at $(0,1)$. It is easy to check that the coalition structure is stable with respect to single-agent, merge, and 2-compromise transitions, but a compromise between the three current coalitions leads to a bigger coalition of size $5$ with a proposal at $(0,1)$ and with players of type $(-1,1)$, $(0,1)$, and $(1,1)$.
\end{enumerate}
The two examples above show that 2-compromise and 3-compromise are necessary for $\bZ_{\ge 0}^2$ grid and $\bZ^2$ grid, respectively. The theorem below proves that they are sufficient.

\begin{theorem}\label{thm:gridOpt}
When the players and the proposals are points in $\bZ_{\ge 0}^2$ and the status quo is at the origin, 2-compromise transitions are sufficient for convergence to an optimal coalition structure. One the other hand, when the players and the proposals are points in $\bZ^2$, and the status quo is at the origin, 3-compromise transitions are sufficient for convergence to an optimal coalition structure.
\end{theorem}

% \begin{theorem}\label{thm:grid3opt}
% When t
% \end{theorem}

We first prove a few useful lemmas that will be used to prove the above theorem. Note that compromise transitions are more general than other kinds of transitions like single-agent or merge, therefore we shall w.l.o.g. only focus on compromise transitions when studying the stability of coalition structures.

\begin{lemma}\label{thm:lemma:gridOpt1}
Let $D$ be a coalition structure. Let $(C,p)$ be a coalition--proposal pair in $D$. Let $p'$ be another proposal such that all players in $C$ also prefer $p'$ than status quo. Let $D'$ be similar to $D$, except that we replace $(C,p)$ by $(C,p')$. We claim that $D'$ is a valid coalition structure, and $D'$ is stable if and only if $D$ is stable.
\end{lemma}
\begin{proof}
$D'$ is a valid coalition structure by construction. As compromise transitions are allowed to select the new proposal where the larger coalition is formed, it is easy to check that a compromise move valid in $D$ is also valid in $D'$, and vice-versa.
\end{proof}

Let the function $sign : \bR \rightarrow \{-1,0,1\}$ be defined as 
\[
    sign(x) = \begin{cases} -1,& \text{ if $x < 0$,} \\
                            0,& \text{ if $x = 0$,} \\
                            1,& \text{ if $x > 0$.}
                \end{cases}
\]
We shall use $d(p,v)$ to denote the grid-distance ($l_1$-distance) between two points $p,v \in \bZ^2$.
\begin{lemma}\label{thm:lemma:gridOpt2}
If a coalition $C$ of players supports a proposal $p = (x,y)$ with $|x| > 1$ or $|y| > 1$, then $C$ also supports $(x-sign(x),y-sign(y))$.
\end{lemma}
\begin{proof}
The operation $(x-sign(x),y-sign(y))$ moves $(x,y)$ towards the origin. There are eight possible cases depending upon $sign(x)$ and $sign(y)$; w.l.o.g., we shall consider the following two cases $(sign(x),sign(y)) = (1,1)$ and $(sign(x),sign(y)) = (1,0)$, the other six cases are symmetric to one of these two.

\textbf{Case 1: $(sign(x),sign(y)) = (1,1)$.} Consider a player $(u,v) \in C$. We know that $(u,v)$ supports $(x,y)$, we need to show that they also support $(x-1,y-1)$. Note that $d((u,v),(0,0)) = |u| + |v| > d((u,v),(x,y)) = |u-x| + |v-y|$. Consider the four possible cases based on the position of $(u,v)$ with respect to $(x,y)$:
\begin{enumerate}
    \item $u < x$ and $v < y$. $d((u,v), (x-1,y-1)) = |(x-1)-u| + |(y-1)-v| = |u-x| + |v-y| - 2 < |u-x| + |v-y| < |u| + |v|$.
    \item $u < x$ and $v \ge y$. $d((u,v), (x-1,y-1)) = |(x-1)-u| + |v-(y-1)| = |x-u| + |v-y| < |u| + |v|$.
    \item $u \ge x$ and $v < y$. Similar argument to the case above.
    \item $u \ge x$ and $v \ge y$. As $x$ and $y$ are greater than $0$, then $u$ and $v$ are also greater than $0$. Also, $x-1\ge 0$ and $y-1 \ge 0$, and as per our original assumption on $(x,y)$, $(x-1,y-1) \neq (0,0)$. So, $d((u,v), (x-1,y-1)) = |u-(x-1)| + |v-(y-1)| = |u| - |(x-1)| + |v| - |(y-1)| < |u| + |v|$.
\end{enumerate}

\textbf{Case 2: $(sign(x),sign(y)) = (1,0)$.} The argument is similar to Case 1. For any $(u,v) \in C$, we have the following two cases:
\begin{enumerate}
    \item $u < x$. $d((u,v), (x-1,y)) = |(x-1)-u| + |v| = |u-x| + |v| - 1 < |u-x| + |v| < |u| + |v|$.
    \item $u \ge x$. As $x > 1$, so $u \ge 1$ and $(x-1) > 0$. We have $d((u,v), (x-1,y)) = |u-(x-1)| + |v| = |u| - |x-1| + |v| < |u| + |v|$.
\end{enumerate}
\end{proof}

\begin{lemma}\label{thm:lemma:gridOpt3}
A player who supports $(1,1)$ also supports $(1,0)$ and $(0,1)$. Similarly, a player who supports $(-1,1)$ also supports $(-1,0)$ and $(0,1)$, who supports $(-1,-1)$ also supports $(-1,0)$ and $(0,-1)$, and who supports $(1,-1)$ also supports $(1,0)$ and $(0,-1)$. Also, a player supports at most one of these four proposals: $(1,1)$, $(1,-1)$, $(-1,1)$, and $(-1,-1)$.
\end{lemma}
\begin{proof}
We prove that a player who supports $(1,1)$, also supports $(1,0)$ and $(0,1)$. A symmetric argument follows for the other three cases. 

Let a player be located at $(u,v)$ and supports $(1,1)$. We claim that $u > 0$ and $v > 0$. Let one of $u$ or $v$ be less than or equal to $0$, w.l.o.g. let $u \le 0$, then $d((u,v),(1,1)) = |u-1|+|v-1| = (|u|+1)+|v-1| \ge (|u|+1)+(|v|-1) = |u|+|v|$. So, the status quo $(0,0)$ is closer or at the same distance as $(1,1)$. Therefore, $(1,1)$ is not supported by $(u,v)$.

As $u>0$ and $v>0$, $d((u,v),(1,0)) = |u-1|+|v| = |u|+|v|-1 < |u|+|v|$ and $d((u,v),(0,1)) = |u|+|v-1| = |u|+|v|-1 < |u|+|v|$. So, $(u,v)$ supports both $(1,0)$ and $(0,1)$.

As we proved that a player $(u,v)$ supports $(1,1)$ implies $u>0$ and $v>0$, with a symmetric argument we also get that $(u,v)$ supports $(1,-1)$ implies $u>0$ and $v<0$, $(u,v)$ supports $(-1,1)$ implies $u<0$ and $v>0$, and $(u,v)$ supports $(-1,-1)$ implies $u<0$ and $v<0$. These four sets of players are disjoint, so any player can support at most one of these four proposals.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:gridOpt}]
We give a constructive proof; starting from any given coalition structure we show how to reach an optimal and stable coalition structure. 

Let us first focus on the $\bZ_{\ge 0}^2$ grid. Let $D$ be a coalition structure. Using Lemma~\ref{thm:lemma:gridOpt2}, we know that any coalition $C$ in $D$ supports at least one of these three proposals $(1,0)$, $(0,1)$, or $(1,1)$, and further using Lemma~\ref{thm:lemma:gridOpt3}, we know that if $C$ supports $(1,1)$ then it also supports $(1,0)$ and $(0,1)$. So, any coalition $C$ in $D$ supports at least one of $(1,0)$ or $(0,1)$, and if $D$ has strictly more than two coalitions, then there will be a merge transition (which is a specific type of 2-compromise). So, when there are no more merge transitions possible, the coalition structure has at most two coalitions.

From Lemmas~\ref{thm:lemma:gridOpt2}~and~\ref{thm:lemma:gridOpt3}, we know that either $(0,1)$ or $(1,0)$ is an optimal proposal (there can be other optimal proposals too). Once there are only two coalitions in the coalition structure, using Lemma~\ref{thm:lemma:gridOpt1}, we can assume that the two coalitions have proposals at either $(1,0)$ or $(0,1)$. In a single 2-compromise, we reach the optimal coalition structure.

The argument for $\bZ^2$ grid is similar. Using Lemmas~\ref{thm:lemma:gridOpt1},~\ref{thm:lemma:gridOpt2},~and~\ref{thm:lemma:gridOpt3}, we can assume that using merge transitions we have reached a coalition structure with at most four coalitions, and one coalition is located at each of the following four proposals: $P = \{(0,1), (1,0), (-1,0), (0,-1)\}$. From Lemmas~\ref{thm:lemma:gridOpt2}~and~\ref{thm:lemma:gridOpt3}, we also know that one of these four proposals in $P$ is an optimal proposal. W.l.o.g., assume that $(0,1)$ is an optimal proposal. Using Lemma~\ref{thm:lemma:gridOpt3}, we know that $(0,1)$ can be supported by the following three types of players depending upon the proposals in $P$ they support: only support $(0,1)$; support $(1,0)$ and $(0,1)$; support $(-1,0)$ and $(0,1)$. All these players are in one of the three coalitions with proposals in $P \setminus \{(0,-1)\}$. So, in a single 3-compromise, we reach an optimal coalition structure. (We get convergence in two more compromises among the remaining coalitions.)
\end{proof}

From the proof above, we also see that there is a sequence of at most $n$ transitions that leads to a stable and optimal coalition structure, where $n$ is the number of players.

==> extra/hypercube.tex <==
\section{Hypercube Deliberation Spaces}\label{sec:hyper}
In this section, we study hypercube deliberation spaces, where the set of proposals $\cX$ is $\{0,1\}^d$, the agents $V$ also lie in $\{0,1\}^d$, $|cV| = n$, and the distance is measured by the Hamming or the Manhattan distance. This models situations where: there is a set of $d$ agendas; each agent either supports or opposes a given agenda; a given proposal approves a subset of the $d$ agendas; the distance between an agent and a proposal is the number of agendas where they disagree.

\subsection{Beyond Two-Way Compromises}
Elkind~et~al.~\cite{elkind2020deliberative} showed that, unlike Euclidean deliberation spaces, $2$-compromise transitions do not guarantee a successful deliberation for hypercube deliberation spaces. They proved the following result:
\begin{theorem}\cite{elkind2020deliberative}\label{thm:kCompromiseOld}
There are hypercube deliberation spaces where $d$-compromise transitions are necessary for a successful deliberation; while, in every hypercube deliberation space, $(2^{d-1} + (d+1)/2)$-compromise transitions are sufficient for a successful deliberation.
\end{theorem}
The result above leaves a big gap between the lower-bound of $d$ and the upper bound of $(2^{d-1} + (d+1)/2)$. We tighten this by proving a lower-bound of $2^{\Theta(d)}$ 

\begin{theorem}\label{thm:expCompHyp}
There are hypercube deliberation spaces where $2^{\Theta(d)}$-compromise transitions are necessary for a successful deliberation.
\end{theorem}
The proof of the above theorem is given in the Appendix. To prove that a $k$-compromise transition is necessary for a successful deliberation, we need to give a deliberation space and a coalition structure, where:
\begin{itemize}
    \item The coalition structure is sub-optimal, i.e., there exists a coalition structure with a larger coalition. One way to prove this is to show that an $\ell$-compromise transition, $\ell \ge k$, from this coalition structure leads to a strictly larger coalition. So, we need to give a particular proposal and a particular set of agents, and argue that these agents support the new proposal, and the new coalition is larger than the current coalitions of all these agents.
    \item Any $\ell$-compromise, for $\ell < k$, does not lead to a strictly larger coalition. First, these must be at least $k$ coalitions in the current coalition structure. Second, we need to prove that for any proposal in the deliberation space, no set of agents from less than $k$ current coalitions that supports this proposal has a size larger than all of their current coalitions.
\end{itemize}
Elkind~et~al.~\cite{elkind2020deliberative} constructed such an example for $k = d$ and proved its correctness. We do this for $k = \binom{(d-1)/9}{(d-1)/27}-1 \ge 3^{(d-1)/27}-1 = 2^{\Theta(d)}$.


\subsection{Complexity of Finding the Optimal Proposal}
In hypercube deliberation spaces, like Euclidean deliberation spaces, finding an optimal proposal is NP-hard, but is fixed parameter tractable if the number of agents $n$ or the number of dimensions $d$ is a constant.

We prove the NP-hardness result by showing that it is NP-complete to decide whether there exists a proposal that is supported by all the agents.\footnote{As a corollary, it is NP-complete to decide whether there is a proposal supported by $\eta \in [n]$ agents. We can prove this by adding another dimension and some dummy agents who never support any proposals that the original set of agents support and vice-versa} Note that for Euclidean deliberation spaces, deciding whether there exists a proposal supported by all the agents is efficiently solvable using linear programs.

\begin{theorem}\label{thm:hypercubeNPHard}
In a hypercube deliberation space, it is NP-complete to decide whether there exists a proposal that is supported by all agents.
\end{theorem}
\begin{proof}[Theorem~\ref{thm:hypercubeNPHard}]
Note that the problem is in NP, because, given a proposal (evidence), we can check for each agent whether it supports the proposal or not. For proving the hardness, we give a reduction from 3-SAT.

For convenience, we shall denote the proposals using the bit-vector notation,  $x \in \cX = \{0,1\}^d$, and the agents using the set notation, $V \subseteq [d]$. Let us denote our problem, deciding the existence of a proposal supported by all agents, as PSAA.

\textit{Characterize PSAA.} Let us give a characterization for the PSAA problem useful for our proof. The distance of the agent $V$ from origin (status quo) is $|V|$. Now, agent $V$ prefers a proposal $x \in \{0,1\}^d$ to origin iff:
\begin{align*}
    \sum_{i \in V} (1-x_i) + \sum_{i \in [d] \setminus V} x_i < |V| \Longleftrightarrow 1 + \sum_{i \in [d] \setminus V} x_i \le \sum_{i \in V} x_i.
\end{align*}
The above inequality is the characteristic inequality of the agent $V$. The inequality above has a special structure: all the $d$ coordinates of $x$ are present either on the left hand side or on the right hand side, with an additional $1$ on the smaller side of the inequality. Every agent enforces an inequality like the one above, and for every inequality of the type above, we can find an agent that enforces it.

\textit{Construction.} We do a reduction from 3-SAT to PSAA, where the 3-SAT is satisfiable iff there is a proposal preferred by all agents.  Let there be a 3-SAT instance with $m$ binary variables. We create an instance of PSAA with $d = 2 m + 7$ dimensions and the number of agents linear in the number of literals. For each binary variable $x_i$ in the 3-CNF formula, let there be two corresponding dimensions in the PSAA, and let the binary values of the proposal along those dimensions be denoted by $x_i$ and $x_i'$, $i \in [m]$. Along the $7$ additional dimensions, let the values be denoted by $\alpha_0, \alpha_1, \alpha_1', \alpha_2, \alpha_2', \alpha_3, \alpha_3'$, and their tuple by $A$.

We add the following constraints on the proposal by creating agents as given below. These constraints are not related to the terms in the 3-CNF formula.
\begin{enumerate}
    \item Set $\alpha = 1$ for all $\alpha \in A$ by adding the following $14$ agents. For $\alpha \in A$, to set $\alpha = 1$, we add $2$ agents as follows:
    \begin{itemize}
        \item $\sum_{i \in [m]} x_i + \sum_{\alpha' \in B} \alpha' + 1 \le \alpha + \sum_{i \in [m]} x_i' + \sum_{\alpha' \in A \setminus B} \alpha'$,
        \item $\sum_{i \in [m]} x_i' + \sum_{\alpha' \in A \setminus B} \alpha' + 1 \le \alpha + \sum_{i \in [m]} x_i + \sum_{\alpha' \in B} \alpha'$,
    \end{itemize}
    where $B$ be a set of any three variables in $A \setminus \{\alpha\}$.
    Adding the two constraints above, we get $\alpha \ge 1 \implies \alpha = 1$. From now on, to simplify notation, we shall write a constraint for an agent using only an odd number of variables among the $7$ variables in $A$, we assume that the remaining even number of variables are equally distributed on the two sides of the inequality and cancel out as they are all $1$. 
    % We can similarly create $2$ constraints each for the other $6$ variables to set them equal to $1$; the main idea is that for $\alpha \in A$, the first agent will have $1$ for $\alpha$, $x_i, i \in [m]$ and $3$ variables in $A \setminus \{\alpha\}$, and $0$ for others, and the second agent will have the vice-versa, except for $\alpha$, which remains $1$.
    \item Set $x_i = x_i'$ for $i \in [m]$ by adding $4 m$ agents. For each $i \in [m]$, we add the following four agents:
    \begin{itemize}
        \item $x_i + \sum_{j \in [m] \setminus \{i\}} x_j + 1 \le \alpha_0 + x_i' + \sum_{j \in [m] \setminus \{i\}} x_j'$
        \item $x_i + \sum_{j \in [m] \setminus \{i\}} x_j' + 1 \le \alpha_0 + x_i' + \sum_{j \in [m] \setminus \{i\}} x_j$
        \item $x_i' + \sum_{j \in [m] \setminus \{i\}} x_j + 1 \le \alpha_0 + x_i + \sum_{j \in [m] \setminus \{i\}} x_j'$
        \item $x_i' + \sum_{j \in [m] \setminus \{i\}} x_j' + 1 \le \alpha_0 + x_i + \sum_{j \in [m] \setminus \{i\}} x_j$
    \end{itemize}
    Using the fact that $\alpha_0 = 1$, from the first two inequalities, we get $x_i \le x_i'$, and from the next two inequalities, we get $x_i' \le x_i$. So, $x_i = x_i'$.
\end{enumerate}

We now add constraints based on the terms in the 3-CNF formula. Let us focus on a term in the 3-SAT, it uses three variables, and let those variables correspond to $i,j,t \in [m]$. Each term can be of four types (the other four types are reducible to these four by renaming $i,j,t$), as enumerated below, and depending upon the type of the term, we give the corresponding constraints for the PSAA instance. For the ease of notation, we shall suppress the variables $(x_{\ell}, \ell \in [m] \setminus \{i,j,t\})$ and $(x'_{\ell}, \ell \in [m] \setminus \{i,j,t\})$ in the constraints below; we have shown that $x_{\ell} = x_{\ell}'$ for all $\ell \in [m] \setminus \{i,j,t\}$, and we can add one element of each pair to the left and the other to the right of the inequality, and they cancel out.
\begin{enumerate}
    \item Term type $(x_i \vee x_j \vee x_t) \equiv x_i + x_j + x_t \ge 1$. We represent this constraint using an agent as follows:
    \begin{multline*}
        1 \le x_i + x_j + x_t \Longleftrightarrow 2 \le 2(x_i + x_j + x_t) \\
        \Longleftrightarrow 1 + \alpha_0 \le (x_i + x_j + x_t) + (x_i' + x_j' + x_t')
    \end{multline*}
    \item Term type $(\neg x_i \vee x_j \vee x_t) \equiv (1-x_i) + x_j + x_t \ge 1$. We represent this as:
    \begin{multline*}
        1 \le (1-x_i) + x_j + x_t \Longleftrightarrow 2(1 + x_i) \le 2(1 + x_j + x_t) \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i) + (x_i') \le (\alpha_1 + \alpha_1') + (x_j + x_t) + (x_j' + x_t')
    \end{multline*}
    \item Term type $(\neg x_i \vee \neg x_j \vee x_t) \equiv (1-x_i) + (1-x_j) + x_t \ge 1$. We represent this as:
    \begin{multline*}
        1 \le (1-x_i) + (1-x_j) + x_t \Longleftrightarrow 2(1 + x_i + x_j) \le 2(2 + x_t) \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i + x_j) + (x_i' + x_j') \le \sum_{\ell \in [2]} (\alpha_{\ell} + \alpha_{\ell}') + (x_t) + (x_t')
    \end{multline*}
    \item Term type $(\neg x_i \vee \neg x_j \vee \neg x_t) \equiv (1-x_i) + (1-x_j) + (1-x_t) \ge 1$. We represent this as:
    \begin{multline*}
        1 \le (1-x_i) + (1-x_j) + (1-x_t) \Longleftrightarrow 2(1 + x_i + x_j + x_t) \le 2(3) \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i + x_j + x_t) + (x_i' + x_j' + x_t') \le \sum_{\ell \in [3]} (\alpha_{\ell} + \alpha_{\ell}')
    \end{multline*}
\end{enumerate}
This completes our construction.

\noindent ``$\Longleftrightarrow$'' It is trivial to check that there is a one-to-one correspondence between an assignment of the variables in a given instance of 3-CNF formula to the variables in the constructed instance of PSAA (because of the constraints $x_i = x_i'$ for $i \in [m]$ and $\alpha = 1$ for $\alpha \in A$). Also, by construction, there is a one-to-one correspondence between that satisfiability of each term in the 3-SAT instance and the constraint in PSAA instance corresponding to that term.
\qed\end{proof}

We now show that the problem of finding an optimal proposal can be done in polynomial-time, if either the number of dimensions $d$ or the number of agents $n$ is a constant. It is also interesting to note that both the algorithms run in a logarithmic time in the non-constant parameter.

\begin{theorem}\label{thm:hypercubeFPT}
In a hypercube deliberation space, if either the number of dimensions $d$ or the number of agents $n$ is a constant, the optimal proposal can be efficiently computed.
\end{theorem}
\begin{proof} 
\textit{Constant number of dimensions.} When $d$ is a constant, then the number of proposals is $2^d$, which is also a constant. So, we can do a brute force search over the proposals. It takes $O(d)$ time to decide whether a given agent prefers a given proposal to status quo. If $n$ is small compared to $2^d$, then the number of agents who support a given proposal can be checked in $O(dn)$ time. While if $n$ is large compared to $2^d$, then multiple agents lie on the same corner-point of the hypercube. If the number of agents at each corner-point of the hypercube is given (each such value uses at most $O(\log n)$ bits), then the number of agents who support a given proposal can be found in $O(d 2^d \log n)$ time. So, overall time complexity is $O(d 2^d \min(n, 2^d \log n) )$.

\textit{Constant number of agents.} When $n$ is a constant, $2^n$ is also a constant. A proposal is a corner point of the $d$-dimensional hypercube, so to find an optimal proposal, we need to select either $0$ or $1$ for each of the $d$ bits of the proposal. Let us arrange the agents in an arbitrary sequence. Given this sequence, let each dimension of the hypercube be associated with a \textit{type}: a characteristic $n$-bit vector indicating the bit-values of the $n$ agents along that dimension. Two dimensions have the same type iff the same set of agents have a bit-value of $1$ along those dimensions. If two dimensions have the same type, then they are identical from our perspective. For a bit vector $\bb = (b_1, \ldots, b_n) \in \{0,1\}^n$, let $n_{\bb}$ denote the number of dimensions of type $\bb$; and for each $\bb$, we need to compute the optimal $x_{\bb} \in \{0\} \cup [n_{\bb}]$ denoting the number of dimensions of this type that are set to $1$ in an optimal proposal. A brute-force algorithm can solve for them in time $O((d/2^n)^{2^n})$; we give a integer linear program (ILP) that does better with respect to the parameter $d$.

Given a subset of agents $S \subseteq \cV$, the following ILP decides whether there is a proposal that is supported by exactly the agents in $S$. It has the following set of constraints:
\begin{enumerate}
    \item For each agent $i$ in $S$,
    \[ \sum_{\bb \mid b_i = 0} x_{\bb} + \sum_{\bb \mid b_i = 1} (n_{\bb} - x_{\bb}) < \sum_{\bb \mid b_i = 1} n_{\bb} \Longleftrightarrow \sum_{\bb \mid b_i = 0} x_{\bb} - \sum_{\bb \mid b_i = 1} x_{\bb} \le -1. \]
    In the constraint above, $\sum_{\bb \mid b_i = 0} x_{\bb}$ counts the number of dimensions where the agent has value $0$, but the proposal has value $1$, while $\sum_{\bb \mid b_i = 1} (n_{\bb} - x_{\bb})$ counts the number of dimensions where the agent has value $1$ but the proposal $0$, overall, it measures the distance of the agent from the proposal. $\sum_{\bb \mid b_i = 1} n_{\bb}$ measures the distance of the agent from the origin (status quo).
    \item For each agent $i$ not in $S$,
    \[ \sum_{\bb \mid b_i = 0} x_{\bb} + \sum_{\bb \mid b_i = 1} (n_{\bb} - x_{\bb}) \ge \sum_{\bb \mid b_i = 1} n_{\bb} \Longleftrightarrow \sum_{\bb \mid b_i = 0} x_{\bb} - \sum_{\bb \mid b_i = 1} x_{\bb} \ge 0. \]
    \item Feasibility constraints, for each $\bb \in \{0,1\}^n$, $0 \le x_{\bb} \le n_{\bb}.$
\end{enumerate}
The ILP above has $2^n$ variables and $n + 2^n$ constraints. Lenstra’s algorithm (and subsequent improvements of it) can solve an ILP in time exponential in the number of variables but linear in the number of bits required to represent the problem (constraints). As $n_{\bb}$ is $O(\log d)$, we get a time complexity of $O(poly(2^{2^n}) \log d)$. We can find the optimal proposal by searching over all $2^n$ subsets of agents $S \subseteq \cV$, the time complexity remains similar $O(2^n poly(2^{2^n}) \log d) = O(poly(2^{2^n}) \log d)$. 
\qed\end{proof}

\subsection{Slow Convergence of Compromise Transitions}
In Section~\ref{sec:euclidSlow}, we gave results that apply to compromise transitions irrespective of the deliberation space. In particular, Theorem~\ref{thm:compromiseUpperBd} and Lemma~\ref{thm:compromiseSlowConverg} apply to hypercube deliberation spaces also.\footnote{Note that $2$-compromise transitions are also $k$-compromise transitions. We can give an upper bound of $k^n$ for $k$-compromise transitions in a manner exactly the same as we did for $2$-compromise transitions in Theorem~\ref{thm:compromiseUpperBd}. For the lower bound, the result for $2$-compromise transitions directly applies to $k$-compromise transitions, although it can be improved slightly for $k$-compromise transitions.} We use Lemma~\ref{thm:compromiseSlowConverg} to prove the following result:
\begin{theorem}
There exist hypercube deliberation spaces where a deliberation may take $\Omega(2^{\sqrt{n}/2})$ $k$-compromise transitions.
\end{theorem}
\begin{proof}
Assume for convenience that $d$ is even (the argument works for odd $d$ with a bit more book-keeping), and let the number of agents $n = d/2$. All these agents have $0$s in their first $d/2$ dimensions and $1$s in all but one (which is different for each agent) of the last $d/2$ dimensions. 

Consider a set $S$ of $m < d/2$ agents. They agree on $(d/2 - m)$ $1$s. Now consider a proposal that has $(d/2 - m - 1)$ $1$s somewhere in the first $d/2$ dimensions and $(d/2 - m)$ $1$s in the dimensions where the agents in $S$ agree on, and $0$s everywhere else. Each agent in $S$ is at a distance of $(d/2-m-1)+ ((d/2-1)-(d/2-m)) = d/2-2$ from this proposal, and at a distance of $d/2-1$ from the origin, so they support the proposal. However, an agent not in $S$ is at a distance of at least $(d/2-m-1) + ((d/2-1)-(d/2-m-2)) = d/2$ from the proposal, so they do not support the proposal.

So, for any subset of agents $S$, there is a proposal that is supported exactly by the agents in $S$. Applying Lemma~\ref{thm:compromiseSlowConverg}, we get the desired result.
\qed\end{proof}

==> extra/hypercubeNPhard.tex <==
% The old proof using 3-SAT. Independent Set proof below.
\iffalse
\begin{proof}
Note that {\sc Perfect Score} is in NP, because, given a proposal, we can check whether each agent approves it. To prove that this problem is NP-hard, we give a reduction from 3-SAT.

It will be convenient to identify proposals with bit vectors in $\{0, 1\}^d$,  
$x \in \cX = \{0,1\}^d$, and agents with subsets of $[d]$, $V \subseteq [d]$. 

We start by giving a characterization of the {\sc Perfect Score} problem that will be useful for our proof. The distance of agent $V$ from the origin (the status quo) is $|V|$. Now, agent $V$ prefers a proposal $x \in \{0,1\}^d$ to the status quo if and only if
\begin{align*}
    \sum_{i \in V} (1-x_i) + \sum_{i \in [d] \setminus V} x_i < |V| \Longleftrightarrow 1 + \sum_{i \in [d] \setminus V} x_i \le \sum_{i \in V} x_i.
\end{align*}
We will refer to the above inequality as the {\em characteristic inequality} of agent $V$. It has a special structure: all the $d$ coordinates of $x$ are present either on the left-hand side or on the right-hand side. There is a one-to-one correspondence between inequalities of this form
and subsets of $[d]$.

We are now ready to present our construction. 
Consider an instance of 3-SAT
with $m$ binary variables. We create a hypercube deliberation space 
with $d = 2 m + 7$ dimensions and $O(m)$ agents
so that the input instance of 3-SAT is satisfiable
if and only if there exists a proposal that is approved by all agents.

We introduce two dimensions for each binary variable $x_i$ in the 3-CNF instance, 
and let the binary values of the proposal along those dimensions be denoted 
by $x_i$ and $x_i'$. Along the $7$ additional dimensions, let the values be denoted by $\alpha_0, \alpha_1, \alpha_1', \alpha_2, \alpha_2', \alpha_3, \alpha_3'$, and their tuple by $A$.

We impose constraints on the proposal by creating agents as described below. The first set of constraints is not related to the terms in the 3-CNF formula.
\begin{enumerate}
    \item For each $\alpha \in A$, we set $\alpha = 1$ by adding $2$ agents as follows. Pick a set $B$ of three variables in $A \setminus \{\alpha\}$, and add agents that correspond to the following inequalities:
    \begin{eqnarray}
        \sum_{i \in [m]} x_i + \sum_{\alpha' \in B} \alpha' + 1 &\le& \alpha + \sum_{i \in [m]} x_i' + \sum_{\alpha' \in A \setminus B} \alpha', \label{eq1}\\
        \sum_{i \in [m]} x_i' + \sum_{\alpha' \in A \setminus B} \alpha' + 1 &\le& \alpha + \sum_{i \in [m]} x_i + \sum_{\alpha' \in B} \alpha'.\label{eq2}
    \end{eqnarray}
    Summing up constraints~\eqref{eq1} and~\eqref{eq2}, we obtain $\alpha \ge 1$ and hence $\alpha = 1$. From now on, to simplify notation, in each constraint we will use an odd number of variables from $A$: the remaining variables in $A$ (an even number of them) can be equally distributed to the two sides of the inequality, and cancel out as they are all $1$. 
    \item For each $i\in [m]$, we set $x_i = x_i'$ by adding $4$ agents as follows:
    \begin{eqnarray}
        x_i + \sum_{j \in [m] \setminus \{i\}} x_j + 1 &\le& \alpha_0 + x_i' + \sum_{j \in [m] \setminus \{i\}} x_j'\label{eq3}\\
        x_i + \sum_{j \in [m] \setminus \{i\}} x_j' + 1 &\le& \alpha_0 + x_i' + \sum_{j \in [m] \setminus \{i\}} x_j\label{eq4}\\
        x_i' + \sum_{j \in [m] \setminus \{i\}} x_j + 1 &\le& \alpha_0 + x_i + \sum_{j \in [m] \setminus \{i\}} x_j'\label{eq5}\\
        x_i' + \sum_{j \in [m] \setminus \{i\}} x_j' + 1 &\le& \alpha_0 + x_i + \sum_{j \in [m] \setminus \{i\}} x_j.\label{eq6}
    \end{eqnarray}
    Using the fact that $\alpha_0 = 1$, from inequalities~\eqref{eq3} and~\eqref{eq4}, we obtain $x_i \le x_i'$, and from~\eqref{eq5} and~\eqref{eq6} we obtain $x_i' \le x_i$. Hence, $x_i = x_i'$.
\end{enumerate}

We now add constraints based on the terms in the 3-CNF formula. 
Consider a term that uses variables $x_i, x_j, x_\ell$.
This term can be of four types (the other four types are reducible to these four by renaming $i,j,\ell$), as enumerated below. and depending upon the type of the term, we give the corresponding constraints for our instance. 
For the ease of notation, we shall suppress the variables 
$(x_t, t \in [m] \setminus \{i,j,\ell\})$ and $(x'_t, t \in [m] \setminus \{i,j,\ell\})$ in the constraints below; we have shown that $x_t = x_t'$ for all $t \in [m] \setminus \{i,j,\ell\}$, and we can add one element of each pair to the left and the other to the right of the inequality, and they cancel out.
\begin{enumerate}
    \item Term type $(x_i \vee x_j \vee x_\ell) \equiv x_i + x_j + x_\ell \ge 1$. We represent this constraint using an agent as follows:
    \begin{eqnarray*}
        1 \le x_i + x_j + x_\ell \Longleftrightarrow 2 \le 2(x_i + x_j + x_\ell) \\
        \Longleftrightarrow 1 + \alpha_0 \le (x_i + x_j + x_\ell) + (x_i' + x_j' + x_\ell').
    \end{eqnarray*}
    \item Term type $(\neg x_i \vee x_j \vee x_\ell) \equiv (1-x_i) + x_j + x_\ell \ge 1$. We represent this as:
    \begin{eqnarray*}
        1 \le (1-x_i) + x_j + x_\ell \Longleftrightarrow 2(1 + x_i) \le 2(1 + x_j + x_\ell) \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i) + (x_i') \le (\alpha_1 + \alpha_1') + (x_j + x_\ell) + (x_j' + x_\ell').
    \end{eqnarray*}
    \item Term type $(\neg x_i \vee \neg x_j \vee x_\ell) \equiv (1-x_i) + (1-x_j) + x_\ell \ge 1$. We represent this as:
    \begin{multline*}
        1 \le (1-x_i) + (1-x_j) + x_\ell \Longleftrightarrow 2(1 + x_i + x_j) \le 2(2 + x_\ell) \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i + x_j) + (x_i' + x_j') \le \sum_{t \in \{1, 2\}} (\alpha_t + \alpha_t') + (x_\ell) + (x_\ell').
    \end{multline*}
    \item Term type $(\neg x_i \vee \neg x_j \vee \neg x_\ell) \equiv (1-x_i) + (1-x_j) + (1-x_\ell) \ge 1$. We represent this as:
    \begin{multline*}
        1 \le (1-x_i) + (1-x_j) + (1-x_\ell) \Longleftrightarrow 2(1 + x_i + x_j + x_\ell) \le 2\cdot 3 \\
        \Longleftrightarrow 1 + \alpha_0 + (x_i + x_j + x_\ell) + (x_i' + x_j' + x_\ell') \le \sum_{t \in [3]} (\alpha_t + \alpha_t').
    \end{multline*}
\end{enumerate}
This completes our construction.

It is immediate that there is a one-to-one correspondence between an assignment of the variables in a given instance of 3-CNF formula to the variables in the constructed instance of {\sc Perfect Score} (because of the constraints $x_i = x_i'$ for $i \in [m]$ and $\alpha = 1$ for $\alpha \in A$). Also, by construction, there is a one-to-one correspondence between satisfying a term in the 3-SAT instance and satisfying the constraint in the instance corresponding to that term.
\end{proof}
\fi
